Efficiently Answering Quality Constrained Shortest Distance Queries in Large Graphs

The shortest-path distance is a fundamental concept in graph analytics and has been extensively studied in the literature. In many real-world applications, quality constraints are naturally associated with edges in the graphs and finding the shortest distance between two vertices $s$ and $t$ along only valid edges (i.e., edges that satisfy a given quality constraint) is also critical. In this paper, we investigate this novel and important problem of quality constraint shortest distance queries. We propose an efficient index structure based on 2-hop labeling approaches. Supported by a path dominance relationship incorporating both quality and length information, we demonstrate the minimal property of the new index. An efficient query processing algorithm is also developed. Extensive experimental studies over real-life datasets demonstrates efficiency and effectiveness of our techniques.

==> sec1_introduction.tex <==
\section{Introduction}
\label{sect:intro}
In graph analytics, the concept of shortest path is critical. Specially, a path between two vertices $s$ and $t$ is shortest if its length is the shortest of all feasible paths between $s$ and $t$. Due to its optimality, shortest paths have been used to tackle a broad range of significant issues, including keyword search~\cite{he2007blinks,jiang2015exact,tao2011nearest}, betweenness centrality~\cite{brandes2001faster,puzis2007fast} and route planning~\cite{abraham2011hub,abraham2012hierarchical}. Given a graph $G$, the length of the shortest paths between $s$ and $t$, i.e., the distance of $s$ and $t$, reflects the vertices' significance in some scenarios. For instance, i) in nearest keyword search, the vertices closest to the query source are favoured~\cite{jiang2015exact}; and ii) in social networks, distances are employed in search ranking to aid users in identifying the most relevant results~\cite{vieira2007efficient}.

In the real-world applications, however, we need a weight constraint for the shortest paths. For instance, in a road network, we demand a shortest path with height permitted for autotrucks. In this scenario, the weight could be the height, thus it is logical to choose a shortest path by which autotrucks could pass. Consequently, this is how we formulate our weight constraint shortest path problem: given a query $s, t$ with a weight constraint $w$, we seek to find a shortest path where each edge has a minimum weight of $w$. 

\stitle{Applications.} Some essential applications are listed as follows:
\begin{figure}[htbp]
\centering
\includegraphics[scale=0.35]{figs/motivation_example_wcspd.eps}
\caption{A Communication Network. $R_i$ indicates the $i^{th}$ router, and $S_i$ indicates the $i^{th}$ switch.}
\label{fig:motivation_wcspd}
\end{figure}


\noindent(1) \underline{\textit{Communication Networks~\cite{qiao2013computing}}}.~To achieve end-to-end Quality-of-Service (QoS) guarantees~\cite{ma1997path}, the transmission of multimedia streams imposes a minimum-bandwidth requirement on all the links on a path. A weight constrained shortest path distance query can determine the shortest path distance between two nodes in a network, where each link has a minimum bandwidth demand of $x$. The resultant path can handle $x$ bits per second for the transmission of a stream, such as audio or video, with a guaranteed bandwidth. The edge weight indicates the bandwidth, and a weight constrained shortest distance (for the consideration of minimum cost or delay) between two locations is demanded such that the passing bandwidth cannot be less than a predetermined threshold. Figure~\ref{fig:motivation_wcspd} illustrates a motivation example. In this figure, some services need a minimum speed guarantee, for example $3$ Mbps. A typical query would be what is the distance from $R_3$ to $R_2$ with such a speed guarantee. In this case, the resultant distance would be $4$ since $R_3 \rightarrow S_1 \rightarrow R_4 \rightarrow S_2 \rightarrow R_2$ fulfills all the criteria, while $R_3 \rightarrow S_1 \rightarrow R_2$ does not owing to speed of $S_1 \rightarrow R_2 = 2$Mbps $<$ $3$ Mbps.

\noindent(2) \underline{\textit{Social Networks~\cite{vieira2007efficient}}}.~In social networks, determining the closeness of two individuals is a critical issue. A popular metric is the distance between them in the social networks, e.g., a 2-hop friendship connection is stronger than a 3-hop one. Nonetheless, such a measure is inappropriate in the scenario below: Numerous vertices have the same distance from the query vertice $q$. Due to the small-world phenomenon, many social network vertices have the same distance. Zhang et al.~\cite{zhang2020hub} propose the shortest path counting to determine the importance of such vertices~\cite{zhang2020hub} based on this reasoning. They disregard the weight of different connections. Weights could indicate the strength of the connections between users, for instance, based on profile similarity and interaction activity~\cite{xiang2010modeling,zhao2012relationship}. In real-world, too weak connections have no effect on the outcomes. To address this research gap, our problem offers a more detailed measurement. To be more precise, the user could query with the weight bound to determine the shortest path distance with all non-weak connections.
% A straightforward method to conduct the online BFS or Dijkstra based search algorithm to answer this queries. Such a method could pruned the unsatisfied weighted-edge, but they could not answer queries in real time. Thus, our index could address this problem with very fast query time, which is helpful in such related applications. The distance query is particularly helpful in estimating the strength between two users in a social network~\cite{li2017experimental}.


\noindent(3) \underline{\textit{Biology Networks~\cite{leser2005query}}}.~Another application for our problem is the biology networks. Pathway queries are vital in the analysis of biological networks, where vertices represent the entities, e.g., enzymes and genes, while edges reflect interactions or relations~\cite{leser2005query}. As shown in~\cite{leser2005query}, one of the four important pathway queries in biological networks is to identify a shortest path between two substances subject to some constraints. The weight could be the activity of kinase~\cite{kitagawa2013activity,biosa2013gtpase}. Consequently, a frequent query in these biology networks is to determine the shortest pathway from substance $u$ to transfer to substance $v$, where all the activities of kinase on this pathway is as least $w$.
% Given two substances s and t, it finds all paths, i.e., chains of interactions, from s to t. In the pathway query language proposed in~\cite{leser2005query}, a hop constraint can be used in the path expression such that users can focus on a limited number of important paths (i.e., interaction chains) between two substances.

% {\color{red}
% \stitle{TODO:} tackle the following problems.
% \begin{itemize}
%     % \item What's the difference with span-reachability? It seems the weight can be considered as the timestamp as well. 
%     \item Investigate if the problem is new.  (done)
%     \item What if we use the methods of label-constraint shortest distance to solve the problem. Need to check the time/space complexities for the methods. (till 09 Dec)
%     \item What is the difference between 2-hop labeling and tree decomposition in indexing shortest distance. 
%     \item widest-path, bottleneck shortest path...
% \end{itemize}
% }


% \stitle{Concerns about This Topic.} 
% \begin{itemize}
%     \item It seems to be hard to make a case study for this topic, and thus the effectiveness of new model/problem may be argued. 
%     \item Need to argue this topic is quite different from the label-constraint shortest distance. In \cite{qiao2013computing}, it use the following two reasons: (1) there is a total order among real-valued weights, but no order among categorical labels. A much more optimized solution can be designed for xxxx by exploiting the total-order property; and  (2) the cardinality of a real-valued weight set is typically much larger than that of a categorical label set. A large weight set can substantially increase the indexing and query complexity of existing methods. 
%     \item If we use 2-hop, the technique may be similar to that of span-reachability. 
% \end{itemize}

% In the aforementioned applications, since such queries are frequently used, a real-time method is demanded. Thus, we investigate the index-based method,

\stitle{Challenges.}~The vast search space and the real-time response time are the primary obstacles of this problem. Since there are numerous queries in real applications, the online search algorithms would face the vast search space and could not answer the queries in real time. As for index-based approach, a na\"ive index approach involves constructing an index for every possible weight $w$. In each constructed graph, pairwise distance information is stored. When a query arrives, we could immediately return the results by the corresponding constructed graph's index. Such a solution could be restricted by the fact that the potential number of $w$ values may be rather large. 
Consequently, such a na\"ive index scheme could not satisfy the requirements in the aforementioned applications. We design a modified 2-hop labeling index for the weight constrained shortest path problem to fill this research gap. To further accelerate indexing time, query time, and to reduce index size, we investigate various pruning rules, propose query-efficient methodology, and produce efficient vertex ordering. 
% Our proposed indexing would be able to meet the needs of the aforementioned applications with all the proposed techniques. In addition, our exhaustive experiments verify the efficiency and effectiveness of our method.

\stitle{Our Approach.}~In this paper, we propose the 2-hop labeling index for the classical shortest path distance problem. Then, for \ourproblem \ problem, we propose a na\"ive 2-hop labeling index as one of baselines. Nevertheless, our index requires \textit{Soundness}, \textit{Completeness}, and \textit{Minimal} characteristics. We investigate the BFS search orders, and proposed a weight- and distance-priority constrained BFS to naturally meet these three features without incurring additional expenses. The three characteristics are proven and fulfilled. Since Query operation is widely used in all phases of this problem, we meticulously design the Query function and achieve $O(|L(s) + L(t)|)$ time complexity by using a nice characteristic of \ourproblem \ problem. Lastly, a hybrid vertex ordering is also proposed to tackle both graphs with small and non-small treewidth. 

\stitle{Contributions.}~Our principal contributions are as follows:
\begin{itemize}
    \item \textit{Theoretical Analysis}.~First, we define the weighted constrained shortest path problem, which has a a variety of applications in light of road networks, social networks, and biological networks. Using two theorems, we analyze the time and space complexity of this problem. In addition, we investigated the \textit{Soundness}, \textit{Completeness}, and \textit{Minimal} characteristics, and proposed a sophisticated index capable of naturally preserving these three desirable features.
    \item \textit{Efficient Index}.~We propose a $2$-hop based index method and examine its \textit{Soundness}, \textit{Completeness}, and \textit{Minimal} characteristics. Both query-efficient method and Distance-Prioritized Traversal Strategy are presented to expedite index construction. Additionally, a hybrid vertex ordering is investigated.
    \item \textit{Comprehensive Experiments.}~Compared to the baselines, our comprehensive experiments demonstrate the efficiency and effectiveness of our proposed method. 
\end{itemize}

\vspace{1mm}
\noindent
{\bf Roadmap.} The rest of the paper is organized as follows. Section~\ref{sect:pre} introduces some preliminaries and Section~\ref{sect:baselines} introduces baselines. Our 2-hop based method is proposed in Section~\ref{sect:index}. Section~\ref{sect:ext} investigates some extension cases, followed by empirical studies in Section~\ref{sect:exp}. Section~\ref{sect:related} surveys important related work. Section~\ref{sect:conclusion} concludes the paper.

%The baseline algorithms should include adjusted BFS and label-constraint shortest path. 

==> sec9_limitations.tex <==
\section{Future works}
\label{sect:limit}

% This subsection discusses future work of this problem in the following.

\noindent \textbf{Maintenance under Dynamic Updates}. Given a graph $G$, a labeling $L(\cdot)$ for $G$ and an update $\Delta G$ to $G$, the problem of dynamic labeling under $\Delta G$ is to maintain $L(\cdot)$ such that the resulting labeling is the corresponding one for $G \oplus \Delta G$, where $G \oplus \Delta G$ is the graph obtained by applying $\Delta G$ to $G$. Since the real-world applications for our problem is naturally dynamic, it is still challenging to achieve high efficiency while maintaining the \textit{Minimal} property.

% For canonical distance labeling, the existing dynamic algorithms all fail to achieve high efficiency while retaining the minimality of the labeling~\cite{akiba2014dynamic,akiba2012shortest,qin2017efficient}, and it is still an open problem regarding how to address this issue. Since our labeling $L \leq (\cdot)$ contains the canonical labeling $L^c_{\leq}(\cdot)$ as a subset, the same challenge persists when designing a dynamic algorithm for $L^c_{\leq}(\cdot)$. Worse yet, the necessity to maintain the information about $\sigma_{v, w}$ can further complicate the design.


% \noindent \textbf{Indexing Size}.~As shown in the experiments, although it could speed up the indexing time by increasing the number of threads. Nevertheless, for some graphs such as DB and FL, our algorithms require far more index space than other graphs of similar size. Unfortunately, thus far it is still not clear what properties of these graphs lead to this inefficiency. Is there an efficiently computable ordering that effectively handles these graphs? Or is the huge resource consumption inevitable even with an optimal ordering under the current
% labeling scheme? Both of the questions are also open.
